Quantum Attacks on Classical Proof Systems - The Hardness of Quantum Rewinding

Quantum zero-knowledge proofs and quantum proofs of knowledge are inherently difficult to analyze because their security analysis uses rewinding. Certain cases of quantum rewinding are handled by the results by Watrous (SIAM J Comput, 2009) and Unruh (Eurocrypt 2012), yet in general the problem remains elusive. We show that this is not only due to a lack of proof techniques: relative to an oracle, we show that classically secure proofs and proofs of knowledge are insecure in the quantum setting. More specifically, sigma-protocols, the Fiat-Shamir construction, and Fischlin's proof system are quantum insecure under assumptions that are sufficient for classical security. Additionally, we show that for similar reasons, computationally binding commitments provide almost no security guarantees in a quantum setting. To show these results, we develop the "pick-one trick", a general technique that allows an adversary to find one value satisfying a given predicate, but not two.

==> macros.tex <==
\makeatletter
\let\OE\undefined
\newcommand\txtrel[1]{\stackrel{\hskip-1in\text{\tiny#1}\hskip-1in}}
\newcommand\eqrefrel[1]{\txtrel{\eqref{#1}}}
\newcommand\starrel{\txtrel{$(*)$}}
\newcommand\tristarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!)$}}
\newcommand\fourstarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!*\!)$}}
\newcommand\starstarrel{\txtrel{$(**)$}}
\newcommand\ok{\mathit{ok}}
\newcommand\bits[1]{\bit^{#1}}
\newcommand\bit{\{0,1\}}
\newcommand\qedbox{\m@th$\Box$}
\newcommand\qedmacro{\hfill\qedbox}
\global\let\qed\qedmacro
\newcommand\skipqed{\global\let\qed\empty}
\newcommand\mathqed{\tag*\qedbox\skipqed}
\newcommand\selfbutter[1]{\ket{#1}\bra{#1}}
\newcommand\inner[2]{\langle#1\vert#2\rangle}
\newcommand\fsq{\tfrac1{\sqrt2}}
\newcommand\pagelabel[1]{\phantomsection\label{#1}}



%
\newcommand\showafter[4]{%
  \ifnum\year>#1\relax
    #4%
  \else
    \ifnum\year=#1\relax
    %
      \ifnum\month>#2\relax
      %
        #4%
      \else
        \ifnum\month=#2\relax
        %
          \ifnum\day>#3\relax
          %
            #4%
          \else
            \ch@removeduplicatespace
          \fi
        \else
          \ch@removeduplicatespace
        \fi
      \fi
    \else
      \ch@removeduplicatespace
    \fi
  \fi}


\declare{macro=\calH, code=\mathcal H, nopage=yes,
  description={Denotes a Hilbert space}}

\declare{macro=\setR, code=\mathbb R, nopage=yes,
  description={Real numbers}}

\declare{macro=\Var, code=\operatorname{Var},
  placeholder=\Var[X], nopage=yes,
  description={Variance of $X$}}

%
%
%

\declare{macro=\poly, code=\mathit{poly}, nopage=yes,
  placeholder=\poly(n),
  description={Polynomially-bounded in $n$}}

%

\declare{macro=\ibit, argspec=[1], code=\mathsf{bit}_{#1},
  placeholder=\ibit i(x),
  description={$i$-th bit of bitstring $x$ (from left)}}

\declare{macro=\im, code=\operatorname{im}, nopage=yes,
  placeholder=\im f,
  description={Image of function $f$}}

\declare{macro=\renyi,  argspec=[1], code=H_{#1},
  placeholder={\renyi\alpha(\calD)},
  description={Renyi entropy of order $\alpha$ of distribution $\calD$}}

%
\declare{macro=\E, code=\operatorname{E}, nopage=yes,
  placeholder=\E[A],
  description={Expected value of random variable $A$}}

\declare{macro=\SD, code=\operatorname{SD},
  placeholder={\SD(A;B)},
  description={Statistical distance between random variables or distributions $A$ and $B$}}

\declare{macro=\TD, code=\operatorname{TD},
  placeholder={\TD(\rho,\rho')},
  description={Trace distance between $\rho,\rho'$. Short
    $\TD(\ket{\Psi},\ket{\Psi'})$
  for 
    $\TD(\selfbutter{\Psi},\selfbutter{\Psi'})$}}


\declare{macro=\floor, argspec=[1], code=\lfloor #1\rfloor, wrap=group,
  placeholder=\floor x, nopage=yes,
  description={$x$ rounded towards $-\infty$}}

\declare{macro=\Sy, argspec=[1], code=S_{#1},
  placeholder=\Sy y,
  description={Set of all ``good'' $x$, in pick-one trick}}

\declare{macro=\ketpsiy, argspec=[1], code=\ket{\Psi(#1)}, wrap=group,
  placeholder=\ketpsiy y,
  description={Superposition of all $x\in\Sy y$, for pick-one trick}}
\newcommand\selfbutterpsiy[1]{\ketpsiy{#1}\bra{\Psi(#1)}}

\declare{macro=\ketpsi, code=\ket{\Sigma\Psi}, wrap=group,
  description={Superposition of all $\ketpsiy y$, for pick-one trick}}
\newcommand\selfbutterpsi{\ketpsi\bra{\Sigma\Psi}}

\declare{macro=\ot, code=\leftarrow,
  placeholder={x\ot A},
  description={$x$ is assigned output of algorithm $A$}}

\declare{macro=\otR, code={\stackrel{\scriptscriptstyle\$}\leftarrow},
  placeholder={x\otR S},
  description={$x$ chosen uniformly from set $S$/according to distribution $S$}}

\declare{macro=\ch, code=\mathit{ch}, wrap=group,
  description={Challenge (second message in sigma-protocol, by
  verifier)}}

\declare{macro=\com, code=\mathit{com}, wrap=group,
  description={Commitment (first message in sigma-protocol, by prover)}}

\declare{macro=\resp, code=\mathit{resp}, wrap=group,
  description={Response (third message in sigma-protocol, by prover})}

%
%
%
%
%
%

\declare{macro=\ellcom, code=\ell_\com,
  description={Length of commitments in sigma-protocol}}
\declare{macro=\ellch, code=\ell_\ch,
  description={Length of challenges in sigma-protocol}}
\declare{macro=\ellresp, code=\ell_\resp,
  description={Length of responses in sigma-protocol}}
\declare{macro=\ellrand, code=\ell_\mathit{rand},
  description={Length of randomness in oracle queries}}

\declare{macro=\ESigma, code=E_\Sigma,
  placeholder={\ESigma},
  description={Special soundness extractor for sigma protocol $\Sigma$}}
\declare{macro=\SSigma, code=S_\Sigma,
  description={Honest-verifier simulator extractor for sigma protocol $\Sigma$}}

\declare{macro=\ket, argspec=[1], code=\lvert#1\rangle, wrap=group,
  placeholder=\ket\Psi,
  description={Vector in a Hilbert space (usually a quantum state)}}

\declare{macro=\bra, argspec=[1], code=\langle#1\rvert, wrap=group,
  placeholder=\bra\Psi,
  description={Conjugate transpose of $\ket\Psi$}}

\declare{macro=\ceil, argspec=[1], code=\lceil#1\rceil, wrap=group,
  placeholder=\ceil x, nopage=yes,
  description={Ceiling ($x$ rounded towards $+\infty$)}}
\newcommand\bceil[1]{\bigl\lceil#1\bigr\rceil}
\newcommand\Bceil[1]{\Bigl\lceil#1\Bigr\rceil}

\declare{macro=\abs, argspec=[1], code=\lvert#1\rvert, wrap=group,
  placeholder=\abs x, nopage=yes,
  description={Absolute value / cardinality of $x$}}
\newcommand\babs[1]{\bigl\lvert#1\bigr\rvert}
\newcommand\Babs[1]{\Bigl\lvert#1\Bigr\rvert}

\declare{macro=\ketno, code=\ket{\mathit{no}},
  description={Superposition of no-instances in Grover search}}
\declare{macro=\ketyes, code=\ket{\mathit{yes}},
  description={Superposition of no-instances in Grover search}}

\declare{macro=\norm, argspec=[1], code=\lVert#1\rVert, wrap=group,
  placeholder=\norm x, nopage=yes,
  description={Euclidean norm of $x$}}
\newcommand\bnorm[1]{\bigl\lVert#1\bigr\rVert}
\newcommand\Bnorm[1]{\Bigl\lVert#1\Bigr\rVert}

\declare{macro=\LR, code=L_R,
  description={Language defined by $R$}}

\declare{macro=\mpair, argspec=[2], code={\langle #1,#2\rangle}, wrap=group,
  placeholder=\ok\ot\mpair PV,
  description={Joint execution of $P$ and $V$, $\ok$ is $V$'s output}}


\declare{macro=\calO, code=\mathcal O,
  description={Denotes an oracle}}

\declare{macro=\Oall, code=\mathcal O_\mathit{all},
  description={The oracles $\OE,\OP,\OR,\OS,\OF,\Opsi,\OV$ together}}

\declare{macro=\Opsi, code=\mathcal O_\Psi,
  description={Oracle that provides $\ket\Psi$}}

\declare{macro=\OF, code=\mathcal O_F,
  description={Oracle, mapping $\ket\Psi\to-\ket\Psi$}}

\declare{macro=\OE, code=\mathcal O_E,
  description={Oracle, enabling extraction}}

\declare{macro=\OP, code=\mathcal O_P,
  description={Oracle, enabling honest proofs}}

\declare{macro=\OR, code=\mathcal O_R,
  description={Oracle, membership in relation $R$}}

\declare{macro=\OS, code=\mathcal O_S,
  description={Oracle, enabling simulation}}

\declare{macro=\secpar, code=\eta,
  description={Security parameter}}

\declare{macro=\OV, code=\mathcal O_V,
  description={Oracle, enabling verification}}

\declare{macro=\ORef, code=\mathcal O_\mathrm{Ref},
  description={Oracle, measures $\ketpsi$}}

\declare{macro=\calD, code=\mathcal D, nopage=yes,
  description={Denotes a distribution}}

\declare{macro=\ketbot, code=\ket\bot,
  description={A fixed stated orthogonal to $\ketpsi$}}

\declare{macro=\kk, code=k, wrap=group,
  description={Cardinality of random sets $\Sy y$ (or $\Sy\com$)}}

\declare{macro=\PFS, code=P_\mathit{FS},
  description={Prover of Fiat-Shamir}}
\declare{macro=\VFS, code=V_\mathit{FS},
  description={Verifier of Fiat-Shamir}}


\declare{macro=\PFis, code=P_\mathit{Fis}, wrap=group,
  description={Prover of Fischlin's construction}}
\declare{macro=\VFis, code=V_\mathit{Fis}, wrap=group,
  description={Verifier of Fischlin's construction}}

\declare{macro=\COM, code=\mathrm{COM}, wrap=group,
  description={Commitment scheme from \autoref{def:com}}}
\declare{macro=\COMverify, code=\COM_\mathit{verify}, wrap=group,
  description={Verification algorithm for $\COM$}}

\declare{macro=\fisb, code=b, wrap=group,
  description={Parameter of Fischlin's scheme: length of $H$-outputs}}
\declare{macro=\fisr, code=r, wrap=group,
  description={Parameter of Fischlin's scheme: number of subproofs}}
\declare{macro=\fisS, code=\mathbf{S}, wrap=group,
  description={Parameter of Fischlin's scheme: maximum sum of
    $H$-outputs}}
\declare{macro=\fist, code=t, wrap=group,
  description={Parameter of Fischlin's scheme: number of tries
    performed by prover}}

\declare{macro=\COMstar, code=\mathsf{COM}^*, wrap=group,
  description={A specific cheating commit phase for attacking
    Fischlin's scheme}}
\declare{macro=\COMopenstar, code=\mathsf{COMopen}^*, wrap=group,
  description={A specific cheating open phase for attacking
    Fischlin's scheme}}

%
%
%


%
%
%
%

